Securing 5G OpenRAN with a Scalable Authorization Framework for xApps

The ongoing transformation of mobile networks from proprietary physical network boxes to virtualized functions and deployment models has led to more scalable and flexible network architectures capable of adapting to specific use cases. As an enabler of this movement, the OpenRAN initiative promotes standardization allowing for a vendor-neutral radio access network with open APIs. Moreover, the O-RAN Alliance has begun specification efforts conforming to OpenRAN's definitions. This includes the near-real-time RAN Intelligent Controller (RIC) overseeing a group of extensible applications (xApps). The use of these potentially untrusted third-party applications introduces a new attack surface to the mobile network plane with fundamental security and system design requirements that are yet to be addressed. To secure the 5G O-RAN xApp model, we introduce the xApp Repository Function (XRF) framework, which implements scalable authentication, authorization, and discovery for xApps. We first present the framework's system design and implementation details, followed by operational benchmarks in a production-grade containerized environment. The evaluation results, centered on active processing and operation times, show that our proposed framework can scale efficiently in a multi-threaded Kubernetes microservice environment and support a large number of clients with minimal overhead.

==> background/texfile.tex <==
This section provides the reader with a brief overview of the relevant background on some of the fundamental design components used in the design of the XRF framework. Initially, we provide an overview of the OAuth 2.0 framework, followed by an explanation of access tokens. Then we explain the concept of sidecar proxies (SCPs) which will become relevant during the implementation details in Section~\ref{sec:frmwdsgn}.

\subsection{Open-Authorization 2.0}
OAuth 2.0 is a well-established standard where a service provider delegates authorization and distribution rights to a trusted middle-man entity~\cite{RFC6749}. The main actors in the OAuth 2.0 framework are the service provider, service requester (client), service server, and the authorization server. For the remainder of this paper, we will consider the service provider and the server to be the same entity. Fig.~\ref{fig:backoauth2} presents the overall flow of the framework.
\begin{figure}[h!]
    \centering
    \includegraphics[width=\columnwidth,trim={0cm 0.5cm 0cm 0cm},clip]{figures/backoauth2.pdf}
     \caption{OAuth 2.0 Framework}
     \label{fig:backoauth2}
\end{figure}
A service will start by requesting an access token from the authorization server for a target service. The server will authenticate this request and issue an access token. The service requester will use this token to access the API of the service provider. The provider will validate this request through the authorization server, and if the token is valid, she will respond to the original request with the desired information. 
\subsection{Access Tokens}
The OAuth 2.0 framework~\cite{RFC6749} uses access tokens~\cite{RFC6750} to authorize service requests. These tokens are typically either session tokens or JSON web tokens (JWTs)~\cite{RFC7519}. The two frameworks are depicted in Fig.~\ref{fig:backtokens}.

\begin{figure}[h!]
    \centering
    \begin{subfigure}[t!]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={11.3cm 8.2cm 11.4cm 6.2cm},clip]{figures/backsessionId.pdf}
        \caption[]%
        {{\small Session tokens}}    
        \label{fig:backsessionId}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t!]{0.24\textwidth}  
        \centering 
        \includegraphics[width=\textwidth,trim={11.3cm 9.1cm 12cm 6.23cm},clip]{figures/backjwt.pdf}
        \caption[]%
        {{\small JSON Web Tokens}}    
        \label{fig:backjwt}
    \end{subfigure}
    \vskip\baselineskip
    \caption{Access token mechanisms}
    \label{fig:backtokens}
\end{figure}
For session tokens shown in Fig.~\ref{fig:backsessionId}, the server will create and maintain a log of users and their associated session IDs for subsequent access requests. This mechanism requires the server to perform look-ups to validate access requests. While it is a prevalent authorization method for web servers, it will be challenging to scale and maintain for a microservice deployment.

JWTs, depicted in Fig.~\ref{fig:backjwt}, are more suitable for this purpose. In this case, all the access details for a particular service required in any future request are parameterized in JSON format and signed by the server, forming a JWT. This token is issued to the user and attached to any API call that will require it.

A JWT contains three elements: header, payload, and signature. The elements are Base64 encoded JSON key-value pairs. The header contains general information such as signature algorithm (e.g., alg: RS256), unique key id (kid) associated with the service consumer, media type (e.g., typ: JWT). The payload element contains service request-related information: the unique identifier of the intended recipient or the service provider (aud), expiration time of the JWT (exp), issuer (iss) of the JWT (e.g.,  authorization server), access type denoted as scope (e.g.,read, write), unique identifier of the service consumer (sub). The issuer signs the first two elements for the recipient to verify the authenticity of the token. 
\subsection{Sidecar Proxies}
In the design of microservice applications for containerized environments, the concept of sidecar proxies (SCPs)~\cite{EdpriceMsft2022Jun} has become a popular choice for abstracting out certain generic functionalities from the main application. This is depicted in Fig.~\ref{fig:backscp}.

\begin{figure}[h!]
    \centering
    \includegraphics[width=\columnwidth,trim={6.1cm 6.9cm 12.5cm 6.6cm},clip]{figures/backscp.pdf}
     \caption{Sidecar proxy utilization in containerized environments}
     \label{fig:backscp}
\end{figure}

In a Kubernetes environment, where the smallest deployment unit is a pod, a single pod comprises multiple containers. One of these containers is the microservice application which is not exposed to the outside of the pod but is supported by SCP containers. These SCPs provide auxiliary security functionality as well as multiple other reverse proxy services to the primary application such as monitoring and various platform abstractions. The concept of SCPs has also been adopted in 3GPP standardization for 5GC VNFs in Rel.16 as a viable method of enabling inter-VNF communication~\cite{3gpp23501}.

==> expsetup/texfile.tex <==
In this section, we describe our testing environment depicted in Fig.~\ref{fig:expsetup} that was used for the scaling experiments.
\begin{figure}[h!]
    \centering
    \includegraphics[width=\columnwidth,trim={9.3cm 4.9cm 12.5cm, 5.8cm},clip]{figures/infrasetup.pdf}
    \caption{Testbed with Openstack virtual machines hosting a Kubernetes cluster}
    \label{fig:expsetup}
\end{figure}

We have two servers that are running a small-scale Openstack infrastructure. One of the nodes is serving as a controller, networking, and block storage node while the other serves as a compute node with a KVM hypervisor. The nodes used are two Precision 7920 Tower servers with
\begin{itemize}
    \item 2 x Intel Xeon Gold 5218R 2.1GHz CPUs,
    \item 512GB RAM,
    \item 1TB disk space.
\end{itemize}

The Openstack compute node is running a total of 8 virtual machines (VMs) for the HA-Kubernetes cluster constructed through the Ranchers Kubernetes Engine (RKE). Three VMs are control nodes, one VM is a network filing system node and the remaining eight are workers. One of the VMs is a large worker (L-worker) for isolating the XRF server from the client deployments so that all the vCPUs are dedicated to running the server threads. The others are small workers (S-worker). The flavors of the nodes are given in Table.~\ref{tbl:kubclusconf}. 

\begin{table}[ht!]
\vspace{12pt}
\centering
\small\selectfont
\caption{HA Kubernetes cluster VM flavors}
\label{tbl:kubclusconf}
%\renewcommand{\arraystretch}{1.1} % for the vertical padding
%\resizebox{\textwidth}{!}{
\begin{tabular}{|p{0.2\columnwidth}|p{0.15\columnwidth}|p{0.1\columnwidth}|p{0.1\columnwidth}|p{0.1\columnwidth}|}
\hline
Node & Instances & vCPUs & RAM (GB) & Disk (GB) \\\hline
Control  & 3 & 2 & 8 & 40 \\\hline
S-worker  & 7 & 6 & 16 & 80 \\\hline
L-worker  & 1 & 20 & 200 & 80 \\\hline
\end{tabular}
%}
\end{table}




==> frmwdsgn/texfile.tex <==
In this section we describe the design details of our system. First we show how the new XRF entity integrates into the 5G and O-RAN ecosystem to address the threat model in Section~\ref{sec:thrmdl}. Secondly, we dive into the details of the implementation in a production-grade environment. Finally we outline details of the message flow which takes place between the entities.

\subsection{XRF Overview}
Our ultimate goal with this framework is to build a mechanism which will oversee the authentication, authorization and discovery of xApps at a large scale. In the current microservice dominant implementation model, a given xApp will be required to consume the services of other xApps for service-chaining their individual functionalities into a complete application. The XRF framework will facilitate this by servicing the local xApps as a local metadata database and an OAuth2.0 server. Our proposed framework is presented in Fig.~\ref{fig:xrfsysdsgn}. The 5GC and MANO have been abstracted our for brevity.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth,trim={0.3cm 6.4cm 2.2cm 3cm},clip]{figures/xrfframdes.pdf}
    \caption{High-level view of the XRF framework architecture}
    \label{fig:xrfsysdsgn}
\end{figure*}

The XRF is composed of two entities. These are the XRF-client (XRFc) side modules and the XRF-server (XRFs). The XRFc modules operate independently from the primary xApp functionality and carry out preliminary operations prior the instantiation of the xApp. The high-level client flow is depicted in Fig.~\ref{fig:xrfsysdsgn}. 

The XRFs functionality is exposed to the XRFc modules through an HTTP server where individual representational state transfer (REST) API endpoints have been crafted to accommodate the XRFc operations. These include the authentication, xApp registration and discovery, the access token request and token introspection handler endpoints. 
 
Throughout its lifecycle an XRFs will maintain the metadata of the registered xApps within its domain and update these profiles however necessary. It can respond to the incoming xApp discovery requests by querying this database and responding with a list of eligible xApp profiles. It will also perform access enforcement through the distribution of the access tokens where the scope of the access token is determined by an internal permissions matrix which is determined by the XRF to resolve any conflicting access rights. This functionality essentially makes the XRFs an OAuth 2.0 authorization server~\cite{RFC6749} where the XRFc modules have a service requester and owner back and forth flow.

Before an xApp is instantiated and becomes service-ready in the near-RT RIC, the XRFc will mutually authenticate with the XRFs. Following a successful authentication, XRFc will create a metadata profile for the xApp and register this profile with the XRFs. This profile will contain a Universally unique identifier (UUID) which will serve as the xApp instance ID among other fundamental pieces of information. 

At this point, the xApp has been fully registered with the XRFs and is ready to carry out the relevant functionality that it was created to fulfil. To initiate or join the service-chain, a requester-xApp (r-xApp) will need to consume the services provided by a serving-xApp (s-xApp).  

This process is initiated with the XRFc of the r-xApp sending a discovery request to the XRFs for type of s-xApp that is advertising a given service offering in the XRFs database. The XRFs will send back the available list of s-xApps to the XRFc of the r-XApp where final selection will be made for an s-xApp through a UUID. 

The XRFc of the r-xApp will proceed to send an access token request to the XRFs for a specific API consumption of the s-xApp that was chosen. In our framework, the access tokens are JWTs explained in Section~\ref{sec:background}.

Using this token, the r-xApp can now proceed to request services from s-xApps. The XRFc of the s-xApp will perform token validation on any incoming service request through either a self-contained validation, which is when the token is validated by the XRFc,  or assisted validation, where the token is forwarded to the token introspection endpoint of the XRFs for validation. Upon successful validation of the token, the r-xApp and s-xApp can resume communication.

\subsection{Implementation Details}
The implementation of the XRFs and XRFc applications is done in C++20. Both the application servers are running an HTTP server with REST API endpoints crafted using Pistache~\cite{GitHubpi38online}. Pistache is a mature C++ API library which is compatible with OpenAPI~\cite{Hellofro97online}. To make the API accessible, we have first prepared the human-readable YAML files with the OpenAPI 3.0.0 specification and later used the OpenAPI generator to create the template API for the source code and populated it with our custom handlers.

\begin{figure}[b!]
    \centering
    \includegraphics[width=\columnwidth,trim={4cm 8cm 10cm 4.3cm},clip]{figures/impdetails.pdf}
    \caption{Full Kubernetes deployment model with application containers and auxiliary functionality providing SCPs}
    \label{fig:impdetails}
\end{figure}

For handling access tokens, we used a JWT library~\cite{GitHubar4online} which uses OpenSSL as a primary dependency. It provides encoding and decoding of access tokens which can be used for the creation and signing of the token and later on the validation procedures respectively. 

The Kubernetes deployment model is given in Fig.~\ref{fig:impdetails}. It shows the deployment of the xApp and XRFs pods. The former is made up of three containers. The xApp application sits in the pod back-end and communicates with the XRFc SCP through inter-process communication (IPC). The XRFc container is running an HTTP server which is not exposed to the network but is connected to an NGINX~\cite{NGINXRev81online} SCP, which is serving as a back-end reverse proxy. The main use of NGINX in this case is to serve as a secure socket layer (SSL) proxy, to encrypt the HTTP traffic from the XRFc module with TLS 1.3 and expose an HTTPs server to the network using in-house certificates. 

The exact same implementation is mirrored on the XRFs pod where the primary XRFs application is separate from the NGINX SCP. This model of deployment ensures that the microservice application is not burdened with any third-party security features which are offloaded into the SCP.

\subsection{XRFs - XRFc Detailed Information Flow}
The first set of messages exchanged between the XRFc and the XRFs are shown in Fig.~\ref{fig:xrfc_s_prelim} starting with the instantiation of the XRFc until it becomes service ready after obtaining an access token for consuming services from other XRFc modules of other xApps. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=\columnwidth,trim={0cm 0.5cm 0cm 0cm},clip]{figures/xrfc_s_prelim.pdf}
    \caption{Preliminary operation flow between XRFc and XRFs showing (1) initial authentication, (2) registration, (3) discovery request, (4) access token request}
    \label{fig:xrfc_s_prelim}
\end{figure}
The first thing that the XRFc will do after being instantiated is authenticate (1) with the XRFs.
%===================================================================================================
%=======================================Sudip's Text================================================
%==============================Detailing the Authentication Process=================================
%===================================================================================================
XRFc generates a random number $m$ and signs it with its private key $PR_{XRF_c}$. Then the signature is appended with the random number and encrypted with the XRFs public key $PU_{XRF_s}$ so that only XRFs can read the contents of the challenge. The challenge is then Base64 encoded and sent as a JSON string. Upon receiving the challenge, XRFs decrypts it with its private key $PR_{XRF_s}$ and verifies the signature using XRFc's public key $PU_{XRF_c}$, thereby authenticating XRFc. If the signature is verified, XRFs signs $m$ with its private key $PR_{XRF_s}$ and encrypts it with XRFc's public key $PU_{XRF_c}$ and sends it back to XRFc in Base64 encoded JSON format. XRFc decrypts the contents and authenticates XRFs by verifying the signature.     
Once the authentication is successful, the XRFc will register (2) by sending the required metadata in a PUT request to the XRFs. This includes the instance UUID, name, functionality offering, current status, reachable IP address and the geographical location.

At this point XRFc has concluded the preliminary operations and is ready to become part of the microservice-chain. To proceed, it will query the XRFs for a discovery (3) request for a target xApp which is advertising the required functionality and a desirable location. The XRFs will respond with the available list of profiles and the XRFc will choose one based on which one has the highest remaining capacity.

In order to consume the API of the chosen xApp, the XRFc will create an access token request (4) with the UUID of this target, its own UUID and the scope of the access that it wants from the chosen xApp. If requested scope is allowed on the target xApp, the XRFs will create a JWT using a new public-private RSA key pair. It will sign the JWT with the private key and forward it to the XRFc.

\begin{figure}[h!]
    \centering
    \includegraphics[width=\columnwidth,trim={0cm 0.5cm 0cm 0cm},clip]{figures/xrfc_s_cons.pdf}
    \caption{(5) Service consumption from a target XRFc of another xApp using a token bearer with (6.1) self-contained JWT validation and (6.2) remote token introspection}
    \label{fig:xrfc_s_cons}
\end{figure}

Having received the access token, the XRFc can now request service consumption from the target XRFc of another xApp, which is depcited in Fig.~\ref{fig:xrfc_s_cons}. In this scenario, the "target XRFc" has already authenticated and registered with the XRF while the "new XRFc" has been newly instantiated. The steps are described below.

The access token obtained in step (4) can be attached in the header of the API calls (5) made to the target XRFc of the target xApp. Upon receiving the API request, the target xApp can utilize two well-known methods of validating the token (6).

\textbf{(6.a) Self-contained JWT validation:} The target XRFc will extract the key id from the header of the JWT and query the XRFs JSON web key set (JWKS) endpoint of the XRFs with this value. This key id will be internally mapped to the public key of the private key used in signing the JWT. The XRFs will respond with this public key and the target XRFc will cache it for future API calls with the same key id. It will then proceed to the validate the token. The advantage of this approach is that after the first API call, the target XRFc can perform validation on the same key id independently from the server. However, this approach expects token validation functionality to be implemented.

\textbf{(6.b) Remote token introspection:} The target XRFc will extract the JWT from the header of the HTTP request and forward it entirely to the XRFs where the latter will validate it in the same way.

Once the token has been validated, the target xApp can now respond (7) to the new xApp with the requrested resource. 

\begin{comment}
\begin{enumerate}
    \item The first thing that the XRFc will do after being instantiated is authenticate with the XRFs. 
%Sudip's text
    \item Once the authentication is successful, the XRFc will register by sending the required metadata in a PUT request to the XRFs. This includes the instance UUID, name, functionality offering, current status, reachable IP address and the geographical location.
    \item At this point XRFc has concluded the preliminary operations and is ready to become part of the microservice-chain. To proceed, it will query the XRFs with a target xApp which is advertising the required functionality and a desirable location. The XRFs will respond with the available list of profiles and the XRFc will choose one based on which one has the highest remaining capacity.
    \item In order to consume the API of the chosen xApp, the XRFc will create an access token request with the UUID of this target, its own UUID and the scope of the access that it wants from the chosen xApp and send it to the XRFs. If request scope is allowed on the target xApp, the XRFs will create a JWT using a new public-private RSA key pair. It will sign the JWT with the private key and forward it to the XRFc.
    \item The XRFc can now attach this JWT in the header of the API calls made to the target XRFc of the target xApp (i.e., XRFc-2). 
    \item Upon receiving the API request, XRFc-2 can utilize two well-known methods of validating the token.
    \begin{enumerate}
        \item \textbf{Self-contained JWT validation:} The target XRFc will extract the key id from the header of the JWT and query the XRFs JSON web key set (JWKS) endpoint of the XRFs with this value. This key id will be internally mapped to the public key of the private key used in signing the JWT. The XRFs will respond with this public key and the target XRFc will cache it for future API calls with the same key id. It will then proceed to the validate the token. The advantage of this approach is that after the first API call, the target XRFc can perform validation on the same key id independently from the server. However, this approach expects token validation functionality to be implemented. 
        \item \textbf{Remote token introspection:} The target XRFc will extract the JWT from the header of the HTTP request and forward it entirely to the XRFs where the latter will validate it in the same way.
    \end{enumerate}
    \item Once the token has been validated, the target xApp can now respond to the new xApp with the requrested resource. 
\end{enumerate}
\end{comment}

















==> introduction/texfile.tex <==
The deployment of the next generation of mobile networks is underway and quickly gaining momentum. These 5G networks will be servicing a wide range of use cases with versatile demands and specific quality of service (QoS) requirements. 

To sustain such a system, offerings will be carried out over logically isolated set of radio access and compute resources denoted as network slices within the 5G ecosystem. Each network slice will be specifically tailored to support different use cases such as enhanced mobile broadband (eMBB), ultra reliable low latency communication (URLLC), massive internet of things (mIoT) and a larger selection of customized slice service types (SST)~\cite{3gpp23501} created by mobile virtual network operators (MVNOs). 

To enable a flexible deployment of the 5G radio access networks (RAN) and the 5G core (5GC), mobile network functions which existed as physical networks functions on proprietary hardware in the previous generation, now embrace the microservice model to be implemented as virtual network functions (VNFs) on commercial off-the-shelf (COTS) servers. 

Furthermore, the legacy implementations of the RAN featured black-box, bulky entities where the radio protocol stack is fully implemented at every unit, which became a limiting factor in expanding the network. To encourage sustainable scalability, numerous open-source projects have dedicated themselves to enabling collaborative growth in the 5G research community. The foremost among these efforts is the OpenRAN initiative lead by the O-RAN Alliance~\cite{ORANALLI41online,9579445}. 

O-RAN proposes the disaggregation and softwarization of the RAN by employing a functionality split in the protocol stack where different virtualized logical entities host different layers of the radio stack at different physical locations~\cite{3gpp38801}. Furthermore, by steering the 5G deployment effort towards the adoption of open source RAN interfaces with standardized APIs, it promotes a vendor neutral integration of the 5G RAN that will allow improvement efforts from multiple communities to seamlessly come together. This collaboration will accelerate the delivery of the infrastructure necessary to support the versatility that 5G networks need.
 
While aiming to achieve such a deployment, O-RAN is committed to remain compliant with the 5G standardization carried out by the 3rd Generation Partnership Project (3GPP). With that in mind, the O-RAN community has its own set of technical specifications outlining the details of the architecture and working groups dedicated to specific areas of development~\cite{oranwg1archdesc}. 

Arguably, one of the more attractive development efforts within O-RAN is the introduction of the near real-time RAN Intelligent Controller (near-RT RIC) and the closed loop control functionalities that accompany it. The framework uses custom extensible applications (xApps) and service models to allow MVNOs a high degree of freedom in accessing and manipulating information directly in the radio stack in a software-defined manor. Fig.~\ref{fig:highlvl5g} is showing a sample, high level integration of O-RAN into the 5G architecture.

\begin{figure}[h!]
    \centering
    \includegraphics[width=\columnwidth,trim={1cm 8cm 3.cm 5.8cm},clip]{figures/5govhead.pdf}
     \caption{High level overview of the 5G ecosystem with O-RAN augmentation}
     \label{fig:highlvl5g}
\end{figure}

The scenario depicts the 7.2 functionality split adopted by O-RAN in the 5G RAN protocol stack~\cite{3gpp38806}. As a result of this, the first three layers are implemented closer to the fronthaul in the distributed unit (DU) while the upper two layers are closer to the backhaul inside the central unit (CU). Both the DU and CU are softwarized entities deployed at micro-datacentres, made up of COTS hardware. The O-RAN near-real time RIC is deployed at the same hierarchy as the DU given that the xApps will subscribe to information from various radio protocol layers while the management back-end of O-RAN is deployed in the central cloud. Certain 5G core components have been deployed in a more distributed fashion while others have been centralized depending on operational requirements. 

While this does create a very flexible RAN deployment, it also introduces a new threat surface along with raising various system design issues. Given the decentralized and modular nature of 5G networks which will be implemented as microservices, it is impractical to implement bulky, monolithic functionalities in a single VNF. This creates a demand for inter-xApp communication at a large scale which requires secure and efficient execution of cross component authorization and discovery. Currently the software community implementation of the OpenRAN project, supervised primarily by the Linux Foundation, is lacking the necessary security fundamentals to enable a scalable deployment.

%The integration of the near-RT RIC, comprised of many moving parts, into an intricate ecosystem such as 5G requires a thorough fulfillment of fundamental system design principles. First and foremost, the near-RT RIC architecture must deliver a scalable and flexible system which can be seamlessly plugged into the relevant components of the 5G network whilst handling the novel threat surface that will arise.

%To that end, we propose the integration of a new VNF called the xApp repository function (XRF) into the existing 5G architecture, which will be responsible for two distinct classes of operation. Firstly, XRF will serve as a decentralized metadata repository for the xApps and provide a middle-man discovery mechanism facilitating the efficient intra-xApp interactions. Secondly, it will server as an OpenAuthorization 2.0 server and handout access tokens to xApps that wish to consume services from other xApps. Essentially, the functionality of the XRF is analogous to the network functions repository function (NRF) in the 5G core networks adapted for operation among xApps. 

%Secondly, in order to achieve finer-grained control over higher complexity operations, XRF will oversee the inter AF-xApp authorization and discovery by interfacing with the NRF metadata repository in the core network. This development effort aims to instill a scalable authorization and discovery framework between xApps and AFs, where the former can interact in near-real time with the RAN nodes, and latter can plug into desired core component APIs, thereby creating a communication highway between the 5G core control plane and the radio stack. The proposed integration along with the event flow is given in Figure 1.

To that end, we introduce the \textbf{xApp repository function (XRF)}, a new VNF which will provide an authentication, authorization and discovery framework for xApps in the near-RT RIC architecture analogous to the network functions repository function (NRF) in the 5GC. Serving as a decentralized metadata repository, XRF will provide a middle-man discovery mechanism, facilitating the secure and efficient interaction of xApps which seek to consume services from other xApps. 

During its lifecycle, an xApp will be instantiated and register with the XRF. This registration is preceded by the mutual authentication of the xApp with the XRF, after which the former will send pre-determined metadata to the latter, to be used in advertising the service readiness of the xApp. In addition to maintaining xApp metadata, the XRF will serve as an OpenAuthorization (OAuth) 2.0 server and distribute JSON web token (JWT) access tokens to the xApps that register with it, enabling them to consume services from xApps through secure API transactions. 

Our main contribution is the system design and implementation of the XRF entity which includes the modular and independent XRF server-side and the xApp client side libraries that do not require any an internal integration with any existing O-RAN project codebase. Following this, we integrate the server and client into a working Linux Foundation O-RAN Kubernetes cluster with template xApps and measure the operational overhead of employing our framework. 
    







==> relworks/texfile.tex <==
O-RAN oriented research has been growing over the past year as the open-source community continues to evolve enabling real-life experimental work. We summarize O-RAN related industrial and academic efforts under three categories. These are the O-RAN compliant experimental testbeds, high-level security surveys with prototype solutions for various security issues in the O-RAN architecture and finally the O-RAN specification efforts with special attention to the work of the security focus group (SFG). 

\textbf{O-RAN/5G testbeds and experimental work.} While it may not directly be related to security, constructing high fidelity 5G testbeds with RAN nodes which can communicate using the required O-RAN protocols will be crucial for conducting high impact research in the near future.

To that end, an augmentation has been performed~\cite{PublicRe8online} on the srsRAN~\cite{srsRANYo94online} gNB where the node has been fitted with an E2 agent~\cite{orane2gen}. This allows the gNB to interact with the near-RT RIC using the E2AP protocol~\cite{orane2ap}. This effort has enabled a real-life platform for preliminary testing with the near-RT RIC, custom xApps and E2 service models~\cite{orane2sm}. This augmentation is featured in~\cite{10114534770863480842,10114534588643466912} where the authors demonstrate various open-source network slicing capabilities with their custom service models and xApps. Using the same srsRAN augmentation, ~\cite{220513178} features a prototype testbed to demonstrate the signalling operations that take place during communication of a real-life near-RT RIC with a gNB. 

Another large collaboration in the creation of a 5G O-RAN testbed for security testing is lead by the Commonwealth Cyber Initiative~\cite{Commonwe39online} where a stable 5G standalone environment is created for both indoor and outdoor measurements. The testbed is designed for O-RAN compliance to enable the seamless adoption of various machine learning models in the near-RT RIC~\cite{9647461}.
% using the Amari callbox RAN~\cite{AMARICal61online}

Being a LF project, O-RAN has management interfaces which can communicate with the open network automation platform~\cite{HomeONAP85online} (ONAP), a management and orchestration entity designed with a 3GPP-compliant network slicing management system for 5G. Capitalizing on this relationship, ~\cite{200508374} proposes a radio resource management framework while also outlining the end-to-end instantiation of the scheme within an ONAP-ORAN integrated environment. 
Several other 5G testbeds have been constructed~\cite{9771908,9562627,9771860} using popular open-source solutions~\cite{bonati2020open} with the interest of furthering O-RAN related research. For a more comprehensive survey of the open-source development efforts the reader is directed to~\cite{esmaeily2021small}.

\textbf{O-RAN security surveys and prototypes.} Given that the development efforts for O-RAN are in their early stages, it is difficult to ascertain a high fidelity threat surface for the entire architecture. Regardless, there are studies which have dedicated themselves to surveying the existing O-RAN architecture and prototyping various security solutions.

To convey an initial understanding of the internals of the O-RAN architecture, authors of~\cite{220201032} have put together a comprehensive primer. While it mainly focuses on explaining the various workflows and communication interactions involved, there are discussions dedicated to summarizing the work conducted by the O-RAN specifications SFG ~\cite{oransfgprotspec,oransfgreqspec,oransfgthrmdl,oransfgpsectest}.

A security oriented systematic breakdown of the threat surface has been conducted for O-RAN in~\cite{220106080} by identifying the threat vectors of known physical and virtualization layers attacks towards specific entities in the O-RAN architecture. While the authors do provide a good overview, specific system design issues relating to certain sub-components such as xApps have not been analyzed here. 

A less comprehensive security analysis is provided in~\cite{220412227} where in addition to discussing potential threats and actors, certain privacy and mitigation strategies for cloud environments are discussed. In the end, authors have concluded that the security concerns will arise primarily from the interactions of O-RAN with 5G, acknowledging the fundamental issues which need to be addressed in such a large-scale integration. 

A technical study on open fronthaul interface security is conducted in~\cite{10114534654813470080}, where the mandatory security requirements for the management, control, user and synchronization planes are presented. The authors then propose MACsec~\cite{8585421} as a candidate for securing the control user planes between the RAN entities (i.e. DU, CU) where open interfaces are used. Independently, the authors of~\cite{9604996} carry out their own analysis of the O-RAN fronthaul and come to propose MACSec as a preliminary method. However, the authors acknowledge that whilst using MACSec certain performance metrics need to be taken into consideration. 

\textbf{O-RAN specifications.} The O-RAN development has been documented in a series of technical specification documents divided into working groups (WG) given in Table.~\ref{tbl:oranwgs}.

\begin{table}[ht!]
\vspace{12pt}
\centering
\small\selectfont
\caption{O-RAN Working Groups}
\label{tbl:oranwgs}
\begin{tabular}{|p{0.03\textwidth}|p{0.255\textwidth}|}
\hline
WG1 & Use Cases and Overall Architecture \\
WG2 & Non-real-time RIC and A1 Interface \\
WG3 & Near-real-time RIC and E2 Interface \\
WG4 & Open Fronthaul Interfaces \\
WG5 & Open F1/W1/E1/X2/Xn Interface \\
WG6 & Cloudification and Orchestration \\
WG7 & White-box Hardware \\
WG8 & Stack Reference Design \\
WG9 & Open X-haul Transport \\
TIFG & Test and Integration Focus Group \\
SFG & Security Focus Group \\\hline
\end{tabular}
\end{table}

We are primarily interested in the work carried out by the SFG, which is internally divided into the security protocol~\cite{oransfgprotspec}, security requirements~\cite{oransfgreqspec}, test specifications~\cite{oransfgpsectest} and threat modelling and remediation analysis~\cite{oransfgthrmdl} sub-groups.

The O-RAN specific components, interfaces, and technologies extend the attack surface of the 5G system defined by 3GPP. This introduces additional security challenges and risks to consider while implementing these augmented functionalities to the existing 3GPP architecture. In~\cite{oransfgprotspec}, the O-RAN SFG outlines the implementation requirements for security protocols (e.g., SSH, IPSec, TLS) used in O-RAN compliant interfaces. O-RAN interfaces that handle sensitive operations (i.e., authentication, confidentiality, integrity) must support most up-to-date versions of the security protocols, disable insecure ciphers by default, and provide upgrade paths for future releases. O-RAN echoes 3GPP's stance in suggesting cutting down on the number of selectable security parameter options to ensure interoperability. 

The O-RAN SFG is working on specifying high-level security requirements and control mechanisms for O-RAN defined interfaces (e.g., A1, O1, E2) and network functions in~\cite{oransfgreqspec}. However, security requirements for network functions and applications (e.g., O-CU, Near-RT RIC, xApps) maintained by O-RAN are yet to be addressed. O-RAN maintained interfaces must provide basic information security primitives such as confidentiality, integrity, data origin authentication, and secure policy driven privileged access control including password policies for accessing systems, services, and applications. 

Validation methods for testing proper implementation of security protocols (e.g., test setup, procedure, requirements), emulation of attacks, and validating possible mitigation strategies for O-RAN maintained interfaces, components, and services are discussed in~\cite{oransfgpsectest}. O-RAN SFG requires password-based authentication for every management plane protocol to be tested against brute force attacks. Network protocols and interfaces must be tested for robustness against fuzzing and distributed denial of service (DDoS) attacks. However, fundamental security testing and validation guidance such as software components security requirements, open fronthaul security testing, security testing for O-RAN components (e.g., Near-RT RIC, xApps, SMO) are still missing in the current version of the specifications.

The purpose of~\cite{oransfgthrmdl} is threefold. Firstly, roles and responsibilities are identified for maintaining and operating O-RAN systems which also includes prerequisites and assumptions to securely implement and run O-RAN defined components, interfaces, and protocols. Secondly, a threat model is constructed by identifying the threat actors, describing the attack surface, identifying the vulnerabilities and assets, and listing affected components for each threat. Finally, security principles and countermeasures are discussed for the identified threats. 

A recent study summarizes the work done by the O-RAN SFG~\cite{9728862} whilst also taking into consideration certain 5G related concerns mentioned in~\cite{8894379}. Currently it provides a concise overview of the perspective on security from the side of the O-RAN specifications. 

While the O-RAN SFG has taken the preliminary steps towards formulating the new threat surface and identifying certain requirements, the majority of the surface remains unmapped. Additionally, no concrete frameworks have been implemented or proposed to address the lack of fundamental security primitives in inter-xApp communication. To the best of our knowledge, this paper is the first to design, implement and analyze a scalable authentication, authorization and discovery framework for xApps.


==> thrmdl/texfile_sudip.tex <==
O-RAN architecture builds on top of the concepts and standards laid out by 3GPP for added functionalities. However, new functions, open interfaces, use of disaggregated COTS hardware, virtualization, and use of open-source code -- increases the attack surface and can introduce new threats.  Therefore, clearly defining the risks and scope considered for introducing a security element (i.e., XRF) in the O-RAN architecture is crucial. This section describes the threat model we considered for this paper. 
\subsection{Assumptions}
\begin{itemize}
    \item Only O-RAN specific functions and interfaces are considered in the threat model, specifically, interfaces and components in close proximity to xApps. 
    \item The interfaces, agents, and supporting software involved in xApp instantiation and execution use security protocols prescribed by O-RAN SFG. 
    \item XRF is a trusted entity running on a secure physical infrastructure and supported by secure software components (e.g., OS, hypervisor, container).
    \item SMO and MANO are trusted entities. 
\end{itemize}

\subsection{Threat Agents}
A malicious xApp or a group of xApps can register with the xApp management service, subscribe to other legitimate xApps of interest, and start eavesdropping on the A1 and E2 interfaces. [A malicious or compromised O-RU can report fabricated radio information to xApps that are subscribed to it and influence optimization, scheduling, and resource management.]

\subsection{Target}
A malicious xApp can target a cell, a group of UEs, or a specific UE to extract sensitive information (e.g., track user location, infer identification) through A1 and E2 interfaces or influence the target to execute malicious instructions by reporting fabricated radio telemetry. It can also affect the performance or QoS requirements of a RAN node by exploiting resources and thereby, affecting the availability of other services. 
